WalkTheDog: Cross-Morphology Motion Alignment via Phase Manifolds

We present a new approach for understanding the periodicity structure and semantics of motion datasets, independently of the morphology and skeletal structure of characters. Unlike existing methods using an overly sparse high-dimensional latent, we propose a phase manifold consisting of multiple closed curves, each corresponding to a latent amplitude. With our proposed vector quantized periodic autoencoder, we learn a shared phase manifold for multiple characters, such as a human and a dog, without any supervision. This is achieved by exploiting the discrete structure and a shallow network as bottlenecks, such that semantically similar motions are clustered into the same curve of the manifold, and the motions within the same component are aligned temporally by the phase variable. In combination with an improved motion matching framework, we demonstrate the manifold's capability of timing and semantics alignment in several applications, including motion retrieval, transfer and stylization. Code and pre-trained models for this paper are available at https://peizhuoli.github.io/walkthedog.

==> figures/2-manifold.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/2-manifold-fig.pdf}
    \caption{Visualization of the common phase manifold $\Ph$ for the human and dog dataset. We collect samples of $\Ph$ by uniformly sampling the phase variable on each connected component $\Ph_i$ and use PCA to reduce dimension for visualization. Each component is homeomorphic to a circle and is represented in a different color. Semantically similar motions from different characters are clustered into the same component.}
    \label{fig:manifold}
\end{figure*}
